Distributed Object Store Principles of Operation The Case for Intelligent Storage

In this paper we look at the growth of distributed object stores (DOS) and examine the underlying mechanisms that guide their use and development. Our focus is on the fundamental principles of operation that define this class of system, how it has evolved, and where it is heading as new markets expand beyond the use originally presented. We conclude by speculating about how object stores as a class must evolve to meet the more demanding requirements of future applications.

==> Makefile <==
# v0.10 22 April 09 RJP: Created

MAKE=make
PDFLATEX=pdflatex
RTFLATEX=latex2rtf
BIBTEX=bibtex

PAPER=doc
#BIBFILE=$(PAPER).bib

TEXFILES = $(wildcard *.tex)

all: subdirs $(PAPER).pdf

$(PAPER).pdf: $(TEXFILES) $(BIBFILE)
	$(PDFLATEX) $(PAPER)
#	$(BIBTEX) $(PAPER)
#	$(PDFLATEX) $(PAPER)
	$(PDFLATEX) $(PAPER)
#	$(RTFLATEX) $(PAPER)

subdirs:
	$(MAKE) -C fig

clean:
	$(MAKE) -C fig clean 
	/bin/rm -rf auto *.aux *~ *.log *.lot *.lof *.toc *.blg *.bbl *.out

clean-all:\
	clean
	/bin/rm -f $(PAPER).pdf

